Adding Gamma-ray Polarimetry to the Multi-Messenger Era

The last decade has seen the emergence of two new fields within astrophysics: gamma ray polarimetry and GW astronomy. The former, which aims to measure the polarization of gamma rays in the energy range of 10s to 100s of keV, from astrophysical sources, saw the launch of the first dedicated polarimeters such as GAP and POLAR. On the other hand, GW astronomy started with the detection of the first black hole mergers by LIGO in 2015, followed by the first multi messenger detection in 2017. While the potential of the two individual fields has been discussed in detail in the literature, the potential for joint observations has thus far been ignored. In this article, we aim to define how GW observations can best contribute to gamma ray polarimetry and study the scientific potential of joint analyses. In addition we aim to provide predictions on feasibility of such joint measurements in the near future. We study which GW observables can be combined with measurements from gamma ray polarimetry to improve the discriminating power regarding GRB emission models. We then provide forecasts for the joint detection capabilities of current and future GW detectors and polarimeters. Our results show that by adding GW data to polarimetry, a single precise joint detection would allow to rule out the majority of emission models. We show that in the coming years joint detections between GW and gamma ray polarimeters might already be possible. Although these would allow to constrain part of the model space, the probability of highly constraining joint detections will remain small in the near future. However, the scientific merit held by even a single such measurement makes it important to pursue such an endeavour. Furthermore, we show that using the next generation of GW detectors, such as the Einstein Telescope, joint detections for which GW data can better complement the polarization data become possible.

==> Adding Gamma-ray Polarimetry to the Multi-Messenger Era/acronyms.tex <==
\begin{acronym}
\acrodef{AG}[AG]{afterglow}
\acrodef{BAT}[BAT]{Burst Alert Telescope}
\acrodef{BB}[BB]{blackbody}
\acrodef{BBH}[BBH]{binary black hole}
\acrodef{BH}[BH]{black hole}
\acrodef{BNS}[BNS]{binary neutron star}
\acrodef{CR}[CR]{cosmic-ray}
\acrodef{EM}[EM]{electromagnetic}
\acrodef{EOS}[EOS]{equation of state}
\acrodef{FAP}[FAP]{false alarm probability}
\acrodef{FAR}[FAR]{false alarm rate}
\acrodef{GBM}[GBM]{Gamma-ray Burst Monitor}
\acrodef{GCN}[GCN]{Gamma-ray Coordinates Network}
\acrodef{GRB}[GRB]{gamma--ray burst}
\acrodef{GR}[GR]{General Relativity}
\acrodef{GW}[GW]{gravitational wave}
\acrodef{IBIS}[IBIS]{Imager on Board the INTEGRAL Satellite}
\acrodef{IBIS/Veto}[IBIS/Veto]{Veto shield of the Imager on Board the INTEGRAL Satellite}
\acrodef{INTEGRAL}[INTEGRAL]{INTErnational Gamma-Ray Astrophysics Laboratory}
\acrodef{IPN}[IPN]{InterPlanetary Network}
\acrodef{ISGRI}[ISGRI]{INTEGRAL Soft Gamma-Ray Imager}
\acrodef{JEM-X}[JEM-X]{Joint European X-Ray Monitor}
\acrodef{LIGO}[LIGO]{Laser Interferometer Gravitational-Wave Observatory}
\acrodef{MCMC}[MCMC]{Markov Chain Monte Carlo}
\acrodef{NS}[NS]{neutron star}
\acrodef{OMC}[OMC]{Optical Monitoring Camera}
\acrodef{PICsIT}[PICsIT]{PIxellated CsI Telescope}
\acrodef{RAVEN}[RAVEN]{Rapid VOEvent Coincidence Monitor}
\acrodef{SAA}[SAA]{South Atlantic Anomaly}
\acrodef{sGRB}[sGRB]{short gamma-ray burst}
\acrodef{SME}[SME]{Standard Model Extension}
\acrodef{SNR}[SNR]{signal--to--noise ratio}
\acrodef{SPI-ACS}[SPI-ACS]{SPectrometer onboard INTEGRAL - Anti-Coincidence Shield}
\acrodef{SPI}[SPI]{SPectrometer onboard INTEGRAL}
\end{acronym}


==> Adding Gamma-ray Polarimetry to the Multi-Messenger Era/data_macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% generated by template.py, please do not edit directly
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% boilerplate

\def\addVAR#1#2{\expandafter\gdef\csname my@data@\detokenize{#1}\endcsname{#2}}
\def\VAR#1{%
  \ifcsname my@data@\detokenize{#1}\endcsname
    \csname my@data@\detokenize{#1}\expandafter\endcsname
  \else
    \expandafter\ERROR
  \fi
}

% extracted definitions

\addVAR{gw170817.SNR.LIGO_H|round(1)}{18.8}
\addVAR{gw170817.SNR.LIGO_L|round(1)}{26.4}
\addVAR{gw170817.SNR.Virgo|round(1)}{2.0}

